Naive Penalized Spline Estimators of Derivatives Achieve Optimal Rates of Convergence

This paper studies the asymptotic behavior of penalized spline estimates of derivatives. In particular, we show that simply differentiating the penalized spline estimator of the mean regression function itself to estimate the corresponding derivative achieves the optimal L2 rate of convergence.

==> derivative_estimation.tex <==
\subsection{Motivation}
In some cases, emphasis is not necessarily on the mean regression function, but instead on some derivative of the function. For instance, in human growth studies, the first derivative of the function relating height and age gives the speed of growth \cite{muller1988, ramsay2002}. In mechanics, the first and second derivatives of displacement as a function of time give velocity and acceleration respectively. Also, estimates of some derivative of the true function, $f$, are used in plug-in bandwidth selection techniques such as Local Polynomial Regression \cite{wand1994kernel}.

Given the non-parametric model \eqref{eqn:1}, a natural question is how do we estimate some derivative $r$ of $f$?
\subsection{Approaches to Derivative Estimation}
There are two broad approaches used in estimating some derivative of the mean regression function $f$ in \eqref{eqn:1}. One class of methods estimates derivatives by first estimating the true function $f$ and differentiating the estimated function. The other class attempts to estimate derivatives directly from the scatterplot.
\subsubsection{Penalized Splines \& the Naive Estimator}
To estimate the $m^{th}$ derivative of the mean regression function in \eqref{eqn:1}, it's reasonable to take the $r^{th}$ derivative of the penalized spline fit $\hat{f}_{pen}$. \cite{simpkin2013} used multiple penalties to improve the fit of the first derivative of the mean regression function. When using P-Splines, it's straightforward to compute the derivative of $\hat{f}_{pen}$. With equally spaced knots, derivative of B-Spline basis depends on differences in the B-Spline coefficients and lower degree B-Spline basis functions.

Given the B-Spline of order $q$
$$g(x; m) = \sum_{i = 1}^K B_i(x; m)\alpha_i$$
The first derivative of $g$, when the knots are equally spaced is given by
$$g'(x; m) = \sum_{i = 1}^K (m-1)B_i(x, m-1)\Delta \alpha_i / h$$
where $h$ is the common distance between the knots. 
It is therefore straightforward to compute the derivative of $\hat{f}_{pen}(x)$ as
\begin{equation}
    \label{eqn:naive}
    \hat{f}_{pen}'(x) &=& B'^T(x)(B^TB/n + \lambda P_q)^{-1}B^Ty/n
\end{equation}
whee $B'^{T}(x) \in \mathbb{R}^K$ is a vector (scaled) of first derivatives of the B-Spline basis functions. We refer to $\hat{f}_{pen}'$ as the \textit{Naive Estimator} of the first derivative of $f$.
\subsubsection{Local Polynomial Regression}
Another popular way to smooth a scatterplot $\left\{x_i, y_i\right\}_{i=1}^n$ is Local Polynomial Regression \cite{wand1994kernel}.
    
    Given a non-parametric model in \eqref{eqn:1}, a local polynomial regression estimates $f(x_i)$ using Kernel $K$ and bandwidth $h$ by Weighted Least Squares with weights given by the density of the Kernel at each point $x_j$, $1\le j \le n$.
    
    Let $\bm{y}=\left(y_1, \dots, y_n\right)^T$ be a vector of responses, and define
    $$ \bm{X_x} = \begin{bmatrix}
    1 & x_1-x & \hdots & (x_1-x)^p\\
    \vdots & \vdots & \ddots & \vdots \\
    1 & x_n - x & \hdots & (x_n-x)^p
    \end{bmatrix} $$
    $$\bm{W_x} = diag\{K_h(x_1-x), \dots, K_h(x_n-x)\}$$
    
    Using Weighted Least Squares (WLS) with design matrix $\bm{X_x}$ and weight matrix $\bm{W_x}$,
    
    \begin{equation}
        \hat{f}_h(x_i) = \bm{e_1^T(X_x^TW_xX_x)^{-1}X_x^TW_xy}
    \end{equation}
    is the local polynomial estimate of $f(x_i)$ of degree $p$ and bandwidth $h$.
    $\bm{e_1}\in \mathbb{R}^{p+1}$ is a vector with first element of 1 and zeros everywhere.
    Thus, $\hat{f}_h(x_i)$ is the intercept of the weighted least squares solution $\bm{\hat{\beta}=(X_x^TW_xX_x)^{-1}X_x^TW_xy}$. It's important to note that $\hat{f}_h(x_i)$ heavily depends on $h$ which controls the amount of smoothing of the estimator. A large value of $h$ results in more smoothing while smaller values result in less smoothing. 
    
    To estimate some $m^{th}$ derivative of $f$, $f^{(m)}(x)$, it's natural to use the intercept term of the $m^{th}$ derivative of the local polynomial being fitted, for $m \le p$. 
    This is given by:
    \begin{equation}
        \hat{f}^{(m)}_h(x_i) = m!\bm{e_{m+1}^T(X_x^TW_xX_x)^{-1}X_x^TW_xy}
    \end{equation}
    where $\bm{e_{m+1}} \in \mathbb{R}^{p+1}$ is a vector with $(m+1)^{th}$ element of 1 and zeros everywhere.
\subsubsection{Empirical Derivatives}
Unlike the Naive Estimator and Local Polynomial Regression Estimator, empirical derivative methods seek to estimate the derivative of $f$ directly without first estimating $f$ itself. This is usually achieved by approximating the derivative from the scatterplot data and using the approximated data to model the derivative.
For instance, \cite{brabanter2013} defined the estimated $m^{th}$ derivative of $f$ as
\begin{equation}
    f_i^{(m)}=\sum_{j=1}^{k_m}w_{j, m} \left(\frac{Y_{i+j}^{(m-1)}-Y_{i-j}^{(m-1)}}{x_{i+j}-x_{i-j}}\right)
\end{equation}
where the weights $w_{j,m}$ are chosen to minimize the variance of the estimator for $m=1$ and intuitively for $m\ge 2$.
\cite{daitong2016} used the estimator
\begin{equation}
    DY_i = \sum_{k=0}^r d_kY_{i+k},\ \ \ 1\le i \le n-r
\end{equation}
for $f^{'}(x_i)$. The $d_k$'s are chosen to minimize the estimation variance.
\subsubsection{}
